Shape optimization for variational inequalities: the scalar Tresca friction problem

This paper investigates, without any regularization or penalization procedure, a shape optimization problem involving a simplified friction phenomena modeled by a scalar Tresca friction law. Precisely, using tools from convex and variational analysis such as proximal operators and the notion of twice epi-differentiability, we prove that the solution to a scalar Tresca friction problem admits a directional derivative with respect to the shape which moreover coincides with the solution to a boundary value problem involving Signorini-type unilateral conditions. Then we explicitly characterize the shape gradient of the corresponding energy functional and we exhibit a descent direction. Finally numerical simulations are performed to solve the corresponding energy minimization problem under a volume constraint which shows the applicability.

==> Shape_TITRE.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{algorithmic}
\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}

% Used for creating new theorem and remark environments
\newsiamremark{remark}{Remark}
\newsiamremark{hypothesis}{Hypothesis}
\crefname{hypothesis}{Hypothesis}{Hypotheses}
\newsiamthm{claim}{Claim}

% Sets running headers as well as PDF title and authors
\headers{Shape optimization for variational inequalities}{S. Adly, L. Bourdin, F. Caubet, and A. Jacob de Cordemoy}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{Shape optimization for variational inequalities:\\the scalar Tresca friction problem}
%\title{An Example Article\thanks{Submitted to the editors DATE.
%\funding{This work was funded by the Fog Research Institute under contract no.~FRI-454.}}}

% Authors: full names plus addresses.
\author{Samir Adly\thanks{Institut de recherche XLIM. UMR CNRS 7252. Universit\'e de Limoges, France. (\email{samir.adly@unilim.fr}).}
\and Lo\"ic Bourdin\thanks{Institut de recherche XLIM. UMR CNRS 7252. Universit\'e de Limoges, France. (\email{loic.bourdin@unilim.fr}).}
\and Fabien Caubet\thanks{Universit\'e de Pau et des Pays de l'Adour, E2S UPPA, CNRS, LMAP, UMR 5142, 64000 Pau, France. (\email{fabien.caubet@univ-pau.fr})} 
\and Aymeric Jacob de Cordemoy\thanks{Universit\'e de Pau et des Pays de l'Adour, E2S UPPA, CNRS, LMAP, UMR 5142, 64000 Pau, (\email{aymeric.jacob-de-cordemoy@univ-pau.fr})}
}

\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}


%%% Local Variables: 
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End: 

